Comparing AI versus Optimization Workflows for Simulation-Based Inference of Spatial-Stochastic Systems

Model parameter inference is a universal problem across science. This challenge is particularly pronounced in developmental biology, where faithful mechanistic descriptions require spatial-stochastic models with numerous parameters, yet quantitative empirical data often lack sufficient granularity due to experimental limitations. Parameterizing such complex models thus necessitates methods that elaborate on classical Bayesian inference by incorporating notions of optimality and goal-orientation through low-dimensional objective functions that quantitatively capture the target behavior of the underlying system. In this study, we contrast two such inference workflows and apply them to biophysics-inspired spatial-stochastic models. Technically, both workflows are simulation-based inference (SBI) methods. The first method leverages a modern deep-learning technique known as sequential neural posterior estimation (SNPE), while the second is based on a classical optimization technique called simulated annealing (SA). We evaluate these workflows by inferring the parameters of two complementary models for the inner cell mass (ICM) lineage differentiation in the blastocyst-stage mouse embryo. This developmental biology system serves as a paradigmatic example of a highly robust and reproducible cell-fate proportioning process that self-organizes under strongly stochastic conditions, such as intrinsic biochemical noise and cell-cell signaling delays. Our results indicate that while both methods largely agree in their predictions, the modern SBI workflow provides substantially richer inferred distributions at an equivalent computational cost. We identify the computational scenarios that favor the modern SBI method over its classical counterpart. Finally, we propose a plausible approach to integrate these two methods, thereby synergistically exploiting their parameter space exploration capabilities.

==> Manuscript_Organization/Figures_Captions.tex <==
\section*{Figures and captions}

% \graphicspath{{./Manuscript_Graphics/}} % Careful!

% Graphics!

% Fig~\ref{fig1}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 7in, height = 8.75in]{Fig1.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf Visual summary of workflows: AI-MAPE versus SA-SGM.} {\bf [A-D]} Common aspects between both workflows. {\bf [A, B]} Simulation data generation and processing pipelines. Computer simulation involves a representation of the biological system (developing ICM) as a static 2D laminar cell lattice of biochemical reaction volumes coupled via a diffusive signaling molecule (FGF4), and the prescription of a prior distribution over the model parameter space, which together feed the spatial-stochastic simulator. Feature engineering encompasses a series of data transformations: reshaping the simulation trajectories onto a regular time mesh; determining system observables at cell scale from relevant protein count time series (total NANOG, GATA6, and/or FGF4 levels); deciding cell-fate classification at tissue scale based on particular protein count thresholds (\emph{EPI lineage} NANOG $\ge$ 388 and GATA6 $\le$ 329, \emph{PRE lineage} NANOG $\le$ 329 and GATA6 $\ge$ 842, \emph{UND (undifferentiated) lineage} otherwise); constructing pattern score time series ensembles. {\bf [C]} Meta Score. We condense into a sole scalar the success of each sampled parameter vector, with respect to the target system behavior, calculating it on an ensemble of pattern score time series. This serves as a stopping criterion for AI-MAPE, and an exploration-guiding criterion for SA-SGM. {\bf [D]} TEAS and OS. We characterize accuracy and precision of the target developmental behavior by calculating these sample statistics on empirical pattern-score distributions. They also allow us to compare results between both workflows, facilitating the selection of the best or optimal parameter sets. See Methods section for complete details. {\bf [AI-MAPE]} During the simulation data generation, processing, and feature engineering phase, we produce 100 thousand spatial-stochastic trajectories, creating a single pattern-score time series ensemble. During the inference phase, this ensemble of pattern-score time series trains 20 separate ANN replicas, allowing us to obtain several posterior distribution approximations. For each posterior, we calculate its MAPE and from it we generate 50 \emph{de novo} simulations, gathering a fresh pattern-score time series ensemble. To select the optimal MAPE parameter set, we pick the empirical pattern-score distribution with the best (highest) associated meta score. If the previous-round best meta score is larger than or equal to the current-round best meta score, then we stop the workflow; otherwise the current-round best posterior is assigned as the next-round prior (or proposal), iterating the procedure. {\bf [SA-SGM]} During the exploration phase, an annealing scheduler coordinates 100 separate searcher replicas, guiding their first round and first step of parameter space probing by using the prescribed prior distribution. Searchers continue until exhausting 1000 exploring steps, transferring their data into an annealing collector; this collector informs the scheduler about starting locations for the next round of parameter space search. During the exploitation phase, the parameter space dataset (model parameter samples) from all searchers and all rounds is partitioned into hierarchically increasing clusters based on particular meta score thresholds. For each cluster, we calculate its SGM and from it we generate 100 \emph{de novo} simulations, gathering a fresh pattern-score time series ensemble. To select the optimal SGM parameter set, we pick the empirical pattern-score distribution with the best (highest) associated OS.}
\label{fig1}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{fig2}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 4.5in, height = 6.75in]{Fig2.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf ITWT and RTM systems: cell- and tissue-scale stochastic trajectories.} {\bf [A, B]} The ITWT is a wild-type-like model of cell-fate proportioning in the mouse embryo inner cell mass (ICM). {\bf [C, D]} The RTM is a mutant-like model lacking FGF4 signaling (no intercellular communication). {\bf [A, C]} Core GRN interactions (top rows); example stochastic trajectories of intracellular or cell-scale dynamics (bottom rows); only main proteins are shown for each system (NANOG, GATA6, and FGF4). {\bf [B, D]} Basic signaling-topology features (top rows); there are three distinct cell-cell communication modes (autocrine signaling, paracrine signaling, and membrane-level exchange of ligand molecules); example stochastic trajectories of extracellular or tissue-scale dynamics (bottom rows); there are three possible cell fates (Epiblast ``EPI'', Primitive Endoderm ``PRE'', and Undifferentiated ``UND''). Notice the disabled components (gray color) for the RTM compared with the ITWT.}
\label{fig2}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{fig3}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 5.325in, height = 5.325in]{Fig3.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf Inferred optimal parameter sets for the RTM system.} {\bf [A]} Selection process for the best or optimal parameter sets of the two SA runs (SA\_1 and SA\_2). Statistics of the selection process for the optimal parameter sets of the two AI runs (AI\_1 and AI\_2) are shown for reference. The Time Ensemble Average Score ``TEAS'' (top row) is calculated by restricting the simulation score data to the 32-48~h interval, determining the ensemble 25-50-75 percentiles, and computing separately the time average of these three statistics: $\overline{\alpha}_{25}$, $\overline{\alpha}_{50}$, and $\overline{\alpha}_{75}$. Whiskers (SA) or dashed lines (AI) represent error bars; i.e., average interquartile ranges. Circles (SA) or solid lines (AI) represent average medians. The Optimality Score ``OS'' (bottom row) is calculated from TEAS via the formula $\emph{OS} = \overline{\alpha}_{50}(1-(\overline{\alpha}_{75}-\overline{\alpha}_{25}))$. Crosses highlight the best parameter sets for the SA runs. Notice that naively picking the best possible meta-score (filtering threshold equal to 1) does not directly translate to finding the best actual performance. {\bf [B]} Behavior at tissue scale for all four parameter sets (100-cell grid): the target of 60 PRE cells and 40 EPI cells should be reached and sustained within a time window between 32 and 48 hours. Note approximately equal standard deviations ``$\sigma$'' (inset plot), and similar intra- but distinct inter-method means ``$\mu$'' (main plot). {\bf [C]} Comparison of all four inferred optimal parameter sets: box-and-whisker diagrams for each AI\_1-related one-dimensional marginal posterior distribution are shown as baselines. Boxes cover interquartile ranges (from 25 to 75 percentiles) and show medians (50 percentiles). Whiskers cover ranges from 2.5 to 97.5 percentiles. Parameter values fall under normalized prior ranges. Notice intra-method similarity and inter-method differences. {\bf [D]} Distance matrix contrasting each pair of parameter sets: the parameter value sets are assumed to be elements of an abstract four-dimensional vector space. Notice once again short intra- but large inter-method distances. The L1 metric (normalized between 0\% and 100\%) was used to quantify distances between parameter vectors.}
\label{fig3}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{fig4}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 5.5in, height = 5.5in]{Fig4.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf RTM system. Analysis of inferred model parameter posterior distributions.} {\bf [A]} One- and two-dimensional marginal posterior distributions estimated from AI\_1 run for global reference. Locations of optimal parameter values with respect to prior ranges are shown for each method-run pair. {\bf [B]} One- and two-dimensional marginal posteriors conditioned on best parameter values (only referencing AI\_1 case); other cases are not shown for simplicity. {\bf [C]} Linear correlation coefficients extracted by conditioning AI\_1 posterior distribution (global reference) on every optimal parameter set separately. Note strong linear correlations among all parameter pairs (indicating potential compensatory mechanisms between each other), as well as strong intra- and inter-method agreement of estimated coefficients. Notice also that this calculation is possible because the trained ANN acts as a surrogate of the simulator and directly approximates the AI\_1 posterior; i.e., no additional simulations are required to extract Pearson's correlation coefficients. Despite significant differences among parameter value sets, the AI\_1-related ANN is capable of providing useful correlation information for all methods and runs. {\bf [D]} Sensitivity to value changes for all parameters; AI\_1 posterior conditional on every optimal parameter value set separately. Sensitivity equal to 0\% signifies that any value within its prior range can recover the ideal or target system behavior (while holding all the other parameters fixed). Sensitivity equal to 100\% signifies that the value must fall within a singular parameter bin (histograms were created with 250 bins per dimension). Note moderate sensitivities (25-50\%), and strong intra- but moderate inter-method agreement of estimated coefficients, for the majority of parameter relations. The AI\_1-related ANN predicts strong sensitivities (50-100\%) of both \textit{Nanog}\_NANOG and \textit{Gata6}\_GATA6 for the SA runs, as well as strong sensitivities of both \textit{Gata6}\_NANOG and \textit{Nanog}\_GATA6 for the AI runs, highlighting weak inter-method estimated-coefficient agreement among parameter singletons. No weak sensitivities (0-25\%) are recorded. See Results section for complementary details.}
\label{fig4}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{fig5}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 4.15in, height = 6.225in]{Fig5.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf RTM system. Analysis of estimated marginalized posterior distributions.} {\bf [A]} Comparisons between one- and two-dimensional (diagonal and upper elements) posterior marginals. Distances with respect to reference case ``AI\_1'' between one- and two-dimensional (diagonal and lower elements) posterior marginals are also shown. Distances are normalized between 0\% (minimally divergent histograms) and 100\% (maximally divergent histograms). Note that off-diagonal entries (lower and upper sectors) symmetrically correspond to one another. For upper-triangular entries, we filter histogram regions where probability masses are greater than or equal to 0.25 (arbitrary threshold), and create smooth projections via Gaussian kernel density estimates. {\bf [B, C]} Mean or average distances between each method-run pair. Notice the same synergy as for the comparison of parameter value sets (see Fig~\ref{fig3}): intra-method similarity and inter-method difference. Differences between the optimal parameter sets strongly correlate with differences between the marginalized posteriors. These differences come both from the two distinct posterior inference methods (AI versus SA), and the two distinct selection processes for the best parameter sets (MAPE versus SGM). Distances (shown as percentages) between raw probability vectors were quantified using the Jensen-Shannon metric (base 2). See also Methods and Results sections for additional details.}
\label{fig5}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{fig6}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 5.5in, height = 5.5in]{Fig6.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf Inferred optimal parameter sets for the ITWT system.} {\bf [A, B]} Behavior at tissue scale for all four parameter sets (100-cell grid). Correct cell-fate proportions should be reached and sustained within a time window between 32 and 48 hours for both system configurations separately. Temporal evolution of system dynamics reflects high target-fulfillment performance for all method-run pairs, strong similarities between AI runs, weak similarities between SA runs, and moderate agreement overall. {\bf [A]} The target of 0 PRE cells and 100 EPI cells applies to the configuration without cell-cell communication (nonfunctional signaling). {\bf [B]} The target of 60 PRE cells and 40 EPI cells applies to the configuration with cell-cell communication (functional signaling). {\bf [C]} Selection process for the best or optimal parameter sets of the two SA runs (SA\_L1 and SA\_L2). Statistics of the selection process for the optimal parameter sets of the two AI runs (AI\_L1 and AI\_L2) are shown for reference. Two techniques are used to produce the joint configuration-score data from the two marginal configuration-score time series (L1-norm- and L2-norm-inspired combinations), but calculating TEAS and OS for all method-run pairs requires a common technique: L1 combination is used for simplicity. See Fig~\ref{fig3} caption for definitions of Time Ensemble Average Score ``TEAS'' and Optimality Score ``OS''. Crosses highlight the best parameter sets for the SA runs. Notice that simply taking the naive approach of picking the best possible meta-score (filtering threshold equal to 1) does not directly translate to finding the best actual performance. See also Methods and Results sections. {\bf [D]} Distance matrix contrasting each pair of parameter sets: the parameter value sets are assumed to be elements of an abstract nineteen-dimensional vector space. Notice stronger agreement among AI\_L1, AI\_L2, and SA\_L2 than between SA\_L1 and SA\_L2. The L1 metric (normalized between 0\% and 100\%) was used to quantify distances between parameter vectors.}
\label{fig6}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{fig7}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 6.25in, height = 6.25in]{Fig7.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf ITWT system. Comparison of all four inferred/optimal parameter sets.} Box-and-whisker diagrams for each AI\_L1-related one-dimensional marginal posterior distribution are shown as baselines. See Fig~\ref{fig3}[C] caption for definitions of boxes and whiskers. Parameter values fall under normalized prior ranges. Top row: inferred core GRN interaction parameters (cell-scale dynamics). Bottom row: inferred spatial coupling (tissue-scale dynamics) and initial condition (mRNA-PROTEIN counts) parameters. Notice strong agreement among parameter sets AI\_L1, AI\_L2, and SA\_L2 for predictions of primary core GRN interaction values (top-left panel), but weak agreement for predictions of secondary core GRN interaction values (top-right panel). Note also moderate agreement among all parameter sets for predictions of other values. These differences indicate emergence of potential compensation mechanisms among parameters, highlighting distinct exploitable strategies to achieve the ideal or target system behavior. For example, \textit{Fgf4}\_NANOG (half-saturation threshold for transcriptional activation of \textit{Fgf4} promoter by NANOG) and \textit{Fgf4}\_GATA6 (half-saturation threshold for transcriptional repression of \textit{Fgf4} promoter by GATA6), intuitively, are diametrically associated and should be correlatively adjusted to tightly control FGF4 production. \textit{Fgf4}\_NANOG is significantly higher (weaker) than \textit{Fgf4}\_GATA6 for AI\_L1, AI\_L2, and SA\_L2, but this relation reverses for SA\_L1. See also Results section for additional details.}
\label{fig7}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{fig8}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 6.75in, height = 6.75in]{Fig8.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf ITWT system. Conditional model parameter correlation matrix.} Linear correlation coefficients extracted by conditioning AI\_L1 posterior distribution (global reference) on its own MAPE. Note that this calculation is possible because the trained ANN acts as a surrogate of the simulator and directly approximates the AI\_L1 posterior; i.e., no additional simulations are required to extract Pearson's correlation coefficients. Notice strong linear correlations between \{mRNA, PROTEIN\} and \{\textit{Nanog}\_NANOG, \textit{Gata6}\_GATA6, \textit{Gata6}\_NANOG, \textit{Nanog}\_GATA6\}. The two parameters ``mRNA'' and ``PROTEIN'' display a strong negative linear correlation between themselves, indicating that the AI\_L1-related ANN learnt their complementary interaction: increasing initial \textit{Nanog}-\textit{Gata6} mRNA molecules should be compensated by, proportionally, decreasing initial NANOG-GATA6 protein copies, balancing the initial cellular resources across the tissue. These two parameters strongly influence the initial \textit{Nanog}-\textit{Gata6}-\textit{Fgf4} (three main genes) expression dynamics, as reflected by their reciprocal relations with \textit{Nanog}\_NANOG, \textit{Gata6}\_GATA6, \textit{Gata6}\_NANOG, \textit{Nanog}\_GATA6, \textit{Fgf4}\_NANOG, and \textit{Fgf4}\_GATA6.}
\label{fig8}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{fig9}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 7in, height = 7in]{Fig9.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf ITWT system. Conditional model parameter sensitivity matrix.} Sensitivity to value changes for all parameters; AI\_L1 posterior conditional on its own MAPE. See Fig~\ref{fig4}[D] caption for definition of sensitivity. Note weak sensitivities (0-25\%) for (only diagonal entries) \textit{Gata6}\_A-ERK, \textit{Nanog}\_A-ERK, $\tau_{\textrm{pho},\textrm{ERK}}$, $\tau_{\textrm{pho},\textrm{NANOG}}$, $\tau_{\textrm{doh},\textrm{NANOG}}$, $\tau_{\textrm{d},\textrm{FGF4}}$, $\tau_{\textrm{escape}}$, $\tau_{\textrm{exchange}}$, and $\chi_{\textrm{auto}}$; moderate sensitivities (25-50\%) for \textit{Nanog}\_NANOG, \textit{Fgf4}\_NANOG, mRNA, and PROTEIN. Notice also strong sensitivities (50-100\%) for \textit{Gata6}\_GATA6, \textit{Gata6}\_NANOG, \textit{Nanog}\_GATA6, \textit{Fgf4}\_GATA6, $\tau_{\textrm{doh},\textrm{ERK}}$, and $\tau_{\textrm{d},\textrm{M-FGFR-FGF4}}$. Strong sensitivities reflect low tolerance to value fluctuations, given any other parameter is fixed at corresponding MAPE, for recapitulating the ideal target system behavior.}
\label{fig9}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{fig10}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 4in, height = 6in]{Fig10.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf ITWT system. Analysis of estimated marginalized posterior distributions.} {\bf [A]} Comparisons between one- and two-dimensional (diagonal and upper elements) posterior marginals. Distances with respect to reference case ``AI\_L1'' between one- and two-dimensional (diagonal and lower elements) posterior marginals are also shown. Distances are normalized between 0\% (minimally divergent histograms) and 100\% (maximally divergent histograms). Note that off-diagonal entries (lower and upper sectors) symmetrically correspond to one another. Only primary core GRN motif relations are shown; see S~Fig~\ref{S6_Fig} for extended plot of core GRN motif and S~Fig~\ref{S7_Fig} for complete plot of parameter relations. For upper-triangular entries, we filter histogram regions where probability masses are greater than or equal to 0.25 (arbitrary threshold), and create smooth projections via Gaussian kernel density estimates. {\bf [B, C]} Mean or average distances between each method-run pair. {\bf [C]} Notice the same synergy as for the comparison of parameter value sets; see Fig~\ref{fig6} and Fig~\ref{fig7}: stronger agreement among AI\_L1, AI\_L2, and SA\_L2 than between SA\_L1 and SA\_L2. The differences between the optimal parameter sets strongly correlate with the differences between the marginalized posteriors. These differences come from the two distinct posterior inference methods (AI versus SA), the two distinct selection processes for the best parameter sets (MAPE versus SGM), and the effect of the curse of dimensionality (limited sample sizes of SA runs). Distances (shown as percentages) between raw probability vectors were quantified using the Jensen-Shannon metric (base 2). See also Methods and Results sections for additional details.}
\label{fig10}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{S1_Fig}. % Fig~\ref{fig1}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 7in, height = 7in]{Fig100.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf Comparing MAPE versus SGM for SNPE-inspired workflow.} To illustrate the validity and practicality of the sample geometric median (SGM), we compute it for all the AI-MAPE workflow runs and show it alongside their associated maximum a posteriori probability estimates (MAPEs). {\bf [A]} RTM system: red and purple colors indicate MAPEs, orange and turquoise colors indicate SGMs, for AI\_1 and A1\_2 runs, respectively. {\bf [B-D]} ITWT system: same as [A], but for AI\_L1 and AI\_L2 runs, respectively. {\bf [A-D]} Note that despite some minor variations, SGMs and MAPEs move side by side, trending in parallel overall. We remark that, in general, the separate SGM component values (inferred model parameters) do not necessarily follow the univariate median of their related one-dimensional marginal posteriors; this observation is expected due to co-dependency among the model parameter values. For clarity, comparisons should proceed pairwise: red-orange, and purple-turquoise. See Fig~\ref{fig3}[C] and Fig~\ref{fig7} for additional details.}
\label{S1_Fig}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{S2_Fig}. % Fig~\ref{fig4}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 5.5in, height = 5.5in]{Fig4_Supplement.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf RTM system. Unconditional model parameter correlation and sensitivity matrices.} {\bf [A]} Linear correlation coefficients directly extracted from AI\_1 posterior distribution (global reference). Note weak linear correlations among several parameter pairs (indicating no potential compensatory mechanisms between each other), as well as moderate linear correlations among \textit{Nanog}\_NANOG-\textit{Nanog}\_GATA6 and \textit{Gata6}\_NANOG-\textit{Nanog}\_GATA6. Notice also that this calculation is possible because the trained ANN acts as a surrogate of the simulator and directly approximates the AI\_1 posterior; i.e., no additional simulations are required to extract Pearson's correlation coefficients. {\bf [D]} Sensitivity to value changes for all parameters; unconditional AI\_1 posterior. Sensitivity equal to 0\% signifies that any value within its prior range can recover the ideal or target system behavior (while holding all the other parameters fixed). Sensitivity equal to 100\% signifies that the value must fall within a singular parameter bin (histograms were created with 250 bins per dimension). Note weak (0-25\%) and moderate (25-50\%) sensitivities for all parameter relations. No strong (50-100\%) sensitivities are recorded. {\bf [C, D]} Conditional model parameter correlation and sensitivity matrices. These two panels are only intended for quick reference; see Fig~\ref{fig4}[C, D] for complete details.}
\label{S2_Fig}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{S3_Fig}. % Fig~\ref{fig6}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 5.5in, height = 5.5in]{Fig6_Supplement.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf Comparison at equal number of simulation-inference rounds (R8) of ITWT system features.} {\bf [A, B]} Behavior at tissue scale for all four parameter sets (100-cell grid). Correct cell-fate proportions should be reached and sustained within a time window between 32 and 48 hours for both system configurations separately. {\bf [A]} The target of 0 PRE cells and 100 EPI cells applies to the configuration without cell-cell communication (nonfunctional signaling). {\bf [B]} The target of 60 PRE cells and 40 EPI cells applies to the configuration with cell-cell communication (functional signaling). {\bf [C]} Selection process for the best or optimal parameter sets of the two SA runs (SA\_L1 and SA\_L2). Statistics of the selection process for the optimal parameter sets of the two AI runs (AI\_L1 and AI\_L2) are shown for reference. Two techniques are used to produce the joint configuration-score data from the two marginal configuration-score time series (L1-norm- and L2-norm-inspired combinations), but calculating TEAS and OS for all method-run pairs requires a common technique: L1 combination is used for simplicity. See Fig~\ref{fig3} caption for definitions of Time Ensemble Average Score ``TEAS'' and Optimality Score ``OS''. Crosses highlight the best parameter sets for the SA runs. Notice that naively picking the best possible meta-score (filtering threshold equal to 1) does not directly translate to finding the best actual performance. {\bf [D]} Distance matrix contrasting each pair of parameter sets: the parameter value sets are assumed to be elements of an abstract nineteen-dimensional vector space. Notice stronger agreement among AI\_L1, AI\_L2, and SA\_L2 than between SA\_L1 and SA\_L2. The L1 metric (normalized between 0\% and 100\%) was used to quantify distances between parameter vectors. See Fig~\ref{fig6} for reference.}
\label{S3_Fig}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{S4_Fig}. % Fig~\ref{fig7}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 6.25in, height = 6.25in]{Fig7_Supplement.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf ITWT system. Comparison at equal number of simulation-inference rounds (R8) of inferred/optimal parameter sets.} Box-and-whisker diagrams for each AI\_L1-related one-dimensional marginal posterior distribution are shown as baselines. See Fig~\ref{fig3}[C] caption for definitions of boxes and whiskers. Parameter values fall under normalized prior ranges. Top row: inferred core GRN interaction parameters (cell-scale dynamics). Bottom row: inferred spatial coupling (tissue-scale dynamics) and initial condition (mRNA-PROTEIN counts) parameters. Notice strong agreement among parameter sets AI\_L1, AI\_L2, and SA\_L2 for predictions of primary core GRN interaction values (top-left panel), but weak agreement for predictions of secondary core GRN interaction values (top-right panel). Note also moderate agreement among all parameter sets for predictions of other values. These differences indicate emergence of potential compensation mechanisms among parameters, highlighting distinct exploitable strategies to achieve the ideal or target system behavior. See Fig~\ref{fig7} for reference.}
\label{S4_Fig}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{S5_Fig}. % Fig~\ref{fig9}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 7in, height = 7in]{Fig9_Supplement.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf ITWT system. Conditional model parameter sensitivity matrix.} Sensitivity to value changes for all parameters; AI\_L2 posterior conditional on its own MAPE. Altogether, this result is identical to the conclusion of Fig~\ref{fig9}. Note weak sensitivities (0-25\%) for (only diagonal entries) \textit{Gata6}\_A-ERK, \textit{Nanog}\_A-ERK, $\tau_{\textrm{pho},\textrm{ERK}}$, $\tau_{\textrm{pho},\textrm{NANOG}}$, $\tau_{\textrm{doh},\textrm{NANOG}}$, $\tau_{\textrm{d},\textrm{FGF4}}$, $\tau_{\textrm{escape}}$, $\tau_{\textrm{exchange}}$, and $\chi_{\textrm{auto}}$; moderate sensitivities (25-50\%) for \textit{Nanog}\_NANOG, \textit{Fgf4}\_NANOG, mRNA, and PROTEIN. Notice also strong sensitivities (50-100\%) for \textit{Gata6}\_GATA6, \textit{Gata6}\_NANOG, \textit{Nanog}\_GATA6, \textit{Fgf4}\_GATA6, $\tau_{\textrm{doh},\textrm{ERK}}$, and $\tau_{\textrm{d},\textrm{M-FGFR-FGF4}}$. Strong sensitivities reflect low tolerance to value fluctuations, given any other parameter is fixed at corresponding MAPE, for recapitulating the ideal or target system behavior. See Fig~\ref{fig4}[D] caption for definition of sensitivity.}
\label{S5_Fig}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{S6_Fig}. % Fig~\ref{fig10}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 7in, height = 7in]{Fig101.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf ITWT system. Analysis of estimated marginalized posterior distributions for the (primary and secondary) core GRN motif relations.} Comparisons between one- and two-dimensional (diagonal and upper elements) posterior marginals. Distances with respect to reference case ``AI\_L1'' between one- and two-dimensional (diagonal and lower elements) posterior marginals are also shown. Distances are normalized between 0\% (minimally divergent histograms) and 100\% (maximally divergent histograms). Distances (shown as percentages) between raw probability vectors were quantified using the Jensen-Shannon metric (base 2). Note that off-diagonal entries (lower and upper sectors) symmetrically correspond to one another. For upper-triangular entries, we filter histogram regions where probability masses are greater than or equal to 0.25 (arbitrary threshold), and create smooth projections via Gaussian kernel density estimates. See Fig~\ref{fig10} for reference.}
\label{S6_Fig}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

% Fig~\ref{S7_Fig}. % Fig~\ref{fig10}.
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\includegraphics[width = 7in, height = 7in]{Fig102_Auxiliar.pdf} \centering % Careful! % {2.75, 4, 5, 7.5, 8.75}
\end{adjustwidth} % Careful!
\begin{figure}[hpt!]
\begin{adjustwidth}{-1.75in}{0in} % Careful!
\caption{{\bf ITWT system. Analysis of estimated marginalized posterior distributions: complete plot of parameter relations.} Comparisons between one- and two-dimensional (diagonal and upper elements) posterior marginals. Distances with respect to reference case ``AI\_L1'' between one- and two-dimensional (diagonal and lower elements) posterior marginals are also shown. Distances are normalized between 0\% (minimally divergent histograms) and 100\% (maximally divergent histograms). Distances (shown as percentages) between raw probability vectors were quantified using the Jensen-Shannon metric (base 2). Note that off-diagonal entries (lower and upper sectors) symmetrically correspond to one another. For upper-triangular entries, we filter histogram regions where probability masses are greater than or equal to 0.25 (arbitrary threshold), and create coarse projections via convex hull approximations. See Fig~\ref{fig10} for reference.}
\label{S7_Fig}
\end{adjustwidth} % Careful!
\end{figure}
\clearpage

